Vocabulary Manipulation for Neural Machine Translation

In order to capture rich language phenomena, neural machine translation models have to use a large vocabulary size, which requires high computing time and large memory usage. In this paper, we alleviate this issue by introducing a sentence-level or batch-level vocabulary, which is only a very small sub-set of the full output vocabulary. For each sentence or batch, we only predict the target words in its sentence-level or batch-level vocabulary. Thus, we reduce both the computing time and the memory usage. Our method simply takes into account the translation options of each word or phrase in the source sentence, and picks a very small target vocabulary for each sentence based on a word-to-word translation model or a bilingual phrase library learned from a traditional machine translation model. Experimental results on the large-scale English-to-French task show that our method achieves better translation performance by 1 BLEU point over the large vocabulary neural machine translation system of Jean et al. (2015).

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

SHELL = /bin/sh
MAKE  = make

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files
texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
figfiles += $(wildcard figs/*.tex)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)

######################################################################
# output files
target =main

######################################################################
# make targets
all: pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps

dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
#	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<

%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
#	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi
	pdfcrop --margin "15 15 15 15" main.pdf
#	@-/bin/rm -f ${tmp_files}

long.bib:	all.bib
	./remove-short.pl all.bib > long.bib

######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile


==> tikz-qtree.tex <==
%    tikz-qtree.tex
%    Version 1.2, 20 Apr 2012

%    Copyright (C) 2002, 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.2:
% - level-specific styles (thanks to Andrew Stacey)

% New in version 1.11:
% - make options compatible with standard tikz trees

% New in version 1.1:
% - sideways trees

%% These macros facilitate building up an object recursively before
%% putting it into the input stream.

\newtoks\@result
\def\@call#1#2{\let\@cont=#2\bgroup\@result={}#1}
\def\@return{\global\@result=\@result\egroup\@cont}

\def\@ifequal#1#2{\edef\testa{#1}\edef\testb{#2}\ifx\testa\testb}

%% scan a tree: this just scans a subtree and then puts it onto the
%% input stream

\def\Tree{\@call\@subtree\@Tree}
\def\@Tree{%
%\showthe\@result %debug
\ifpgfpicture % is there a test for tikzpicture?
\pgftree{\the\@result}%
\else
\tikzpicture[baseline]\pgftree{\the\@result}\endtikzpicture
\fi
}

%% scan a subtree
\newtoks\child@list
\newtoks\root@node

\def\@subtree[{%
\root@node={}%
\pgfutil@ifnextchar.{\@call\@interior\@@subtree}{\@@@subtree}}
\def\@@subtree{%
\root@node=\@result
\@@@subtree
}
\def\@@@subtree{%
\@call\@children\@@@@subtree
}
\def\@@@@subtree]{%
\child@list=\@result
\pgfutil@ifnextchar.{\@call\@interior\@@@@@subtree}{\@@@@@@subtree}}
\def\@@@@@subtree{%
%%% Check for mismatch.
\@ifequal{\the\root@node}{\pgfutil@empty}%
  \root@node=\@result
\fi
\@ifequal{\the\root@node}{\the\@result}\else
  \message{Warning: mismatched labels, \the\root@node{} and \the\@result.}%
\fi
\@@@@@@subtree
}
\def\@@@@@@subtree{%
\@ifequal{\the\root@node}{\pgfutil@empty}%
\edef\act{\noexpand\@result={%
\noexpand\subtree@hook
\noexpand\pgfsubtree{\noexpand\path coordinate (\noexpand\nodename);}{\the\child@list}}}%
\else
\edef\act{\noexpand\@result={%
\noexpand\subtree@hook
\noexpand\pgfsubtree{\the\root@node}{\the\child@list}}}%
\fi
\act
\@return}

%% scan a sequence of subtrees or leaves

\newif\ifscanned@edge

\def\@children{%
\scanned@edgefalse
\child@list{}%
\@@children}
\def\@@children{%
\pgfutil@ifnextchar]{\@result\child@list\@return}{% end of children
\pgfutil@ifnextchar\edge{% explicit edge
\ifscanned@edge
\message{Warning: more than one edge given for a single child}\let\next\@@children % ignore
\else
\scanned@edgetrue\let\next\@@@children
\fi
\@call\@edge\next}{%
% else, a real node is next
\ifscanned@edge\else % no explicit edge, supply default
\expandafter\child@list\expandafter{\the\child@list{\edge@adapter{}}}%
\fi
\scanned@edgefalse
\pgfutil@ifnextchar[{% subtree
\expandafter\child@list\expandafter{\the\child@list{\level@hook\interior@hook}}%
\@call\@subtree\@@@children}%
{% leaf
\expandafter\child@list\expandafter{\the\child@list{\level@hook\frontier@hook}}%
\@call\@leaf\@@@children}%
}}}
\def\@@@children{%
% wrap child inside curly braces
\expandafter\@result\expandafter{\expandafter{\the\@result}}%
\edef\act{\noexpand\child@list{\the\child@list \the\@result}}\act
\@@children
}

\def\@interior.{\@result{\node[alias=\nodename][every tree node,every internal node,every level \the\pgftree@level\space node/.try]}\@label}

\def\@leaf{\@call\@label\@@leaf}
\def\@@leaf{\edef\act{\noexpand\@result{%
\noexpand\subtree@hook
\noexpand\pgfsubtree{\noexpand\node[alias=\noexpand\nodename][every tree node,every leaf node,every level \noexpand\the\pgftree@level\space node/.try]\the\@result}{}}}\act\@return}

\def\@edge\edge #1;{%
\@result{\edge@adapter{#1}}%
\@return}
\def\edge@adapter#1{%
\let\tikzparentnode\parentnodename
\let\tikzchildnode\nodename
\path edge from parent #1;%
}

\def\level@hook{%
{\advance\pgftree@level by 1\relax
\xdef\@act{\noexpand\tikzset{level \the\pgftree@level/.try}}}\@act}
\def\subtree@hook{%
%\edef\act{\noexpand\tikzset{every tree node/.append code={\noexpand\tikzset{every level \the\pgftree@level+ node/.try}}}}\act
{\advance\pgftree@level by 1\relax
\xdef\@act{\noexpand\tikzset{level \the\pgftree@level+/.try}}}\@act
}
\def\interior@hook{\tikzset{interior/.try}}
\def\frontier@hook{\tikzset{frontier/.try}}

% a label is either text or PGF/TikZ code starting with \node
\def\@label{\pgfutil@ifnextchar\node{\@litlabel}{\@@label}}
\def\@@label#1 {%
\expandafter\@result\expandafter{\the\@result{#1};}%
\@return}

% try to copy \node command into \@result without stripping braces
\def\@litlabel\node{\@@litlabel}
\def\@@litlabel{\pgfutil@ifnextchar\bgroup{\@@@litlabel}{\@@@@litlabel}}
\def\@@@litlabel#1{\expandafter\@result\expandafter{\the\@result {#1}}\@@litlabel}
\def\@@@@litlabel#1;{\expandafter\@result\expandafter{\the\@result #1;}\@return}

% predefined edges

\def\tree@edge#1#2{(#1.\pgftree@parentanchor) -- (#2.\pgftree@childanchor)}

\def\roof@edge#1#2{\csname roof@edge@\leveldirection\endcsname{#1}{#2}}
\def\roof@edge@down#1#2{(#1.south) -- (#2.north west) -- (#2.north east) -- cycle}
\def\roof@edge@up#1#2{(#1.north) -- (#2.south west) -- (#2.south east) -- cycle}
\def\roof@edge@left#1#2{(#1.west) -- (#2.north east) -- (#2.south east) -- cycle}
\def\roof@edge@right#1#2{(#1.east) -- (#2.north west) -- (#2.south west) -- cycle}

%%% Options
\pgfkeysgetvalue{/tikz/level distance/.@cmd}{\orig@leveldistance}
\tikzoption{level distance}{\pgfmathsetlength\levelsep{#1}\orig@leveldistance#1\pgfeov}
\tikzoption{distance from root}{\pgfmathsetlength\levelsep{#1}\advance\levelsep by -\pgftree@depth}
\pgfkeysgetvalue{/tikz/sibling distance/.@cmd}{\orig@siblingdistance}
\tikzoption{sibling distance}{\pgfmathsetlength\subtreesep{#1}\orig@siblingdistance#1\pgfeov} % different semantics

% I don't really like this scheme
\pgfkeysgetvalue{/tikz/grow/.@cmd}{\orig@grow}
\tikzoption{grow}{\csname grow@#1\endcsname\orig@grow#1\pgfeov}
\pgfkeysgetvalue{/tikz/grow'/.@cmd}{\orig@growprime}
\tikzoption{grow'}{\csname growprime@#1\endcsname\orig@growprime#1\pgfeov}
\def\grow@up{\def\leveldirection{up}\def\siblingdirection{left}}
\def\grow@down{\def\leveldirection{down}\def\siblingdirection{right}}
\def\growprime@up{\def\leveldirection{up}\def\siblingdirection{right}}
\def\growprime@down{\def\leveldirection{down}\def\siblingdirection{left}}
\def\grow@left{\def\leveldirection{left}\def\siblingdirection{down}}
\def\grow@right{\def\leveldirection{right}\def\siblingdirection{up}}
\def\growprime@left{\def\leveldirection{left}\def\siblingdirection{up}}
\def\growprime@right{\def\leveldirection{right}\def\siblingdirection{down}}

% defaults appropriate for linguistic trees
\def\tikz@edge@to@parent@path{\tree@edge{\tikzparentnode}{\tikzchildnode}}
\tikzset{every tree node/.style={anchor=base}}
\tikzset{every leaf node/.style={}}
\tikzset{every internal node/.style={}}

% predefined roof style
\tikzset{roof/.style={edge from parent path=\roof@edge{\tikzparentnode}{\tikzchildnode}}}

